VLSTM: Very Long Short-Term Memory Networks for High-Frequency Trading

Financial trading is at the forefront of time-series analysis, and has grown hand-in-hand with it. The advent of electronic trading has allowed complex machine learning solutions to enter the field of financial trading. Financial markets have both long term and short term signals and thus a good predictive model in financial trading should be able to incorporate them together. One of the most sought after forms of electronic trading is high-frequency trading (HFT), typically known for microsecond sensitive changes, which results in a tremendous amount of data. LSTMs are one of the most capable variants of the RNN family that can handle long-term dependencies, but even they are not equipped to handle such long sequences of the order of thousands of data points like in HFT. We propose very-long short term memory networks, or VLSTMs, to deal with such extreme length sequences. We explore the importance of VLSTMs in the context of HFT. We compare our model on publicly available dataset and got a 3.14\% increase in F1-score over the existing state-of-the-art time-series forecasting models. We also show that our model has great parallelization potential, which is essential for practical purposes when trading on such markets.

==> extras/04-problem_statement.tex <==
\section{Problem Statement}

We aim to create a pipeline which uses past and current snapshots of the order book to predict price movement in the near future and then use this to make trading decision for maximum profitability.

\subsection{Tick Data}
Tick data refers to most granular level market information available from electronically traded markets. Every order request, change in the state of order book and trade information is registered as a "tick" event. State of the order book refers to the top few (five, in our case) bid orders and ask orders currently placed. Tick data is raw, uncompressed data of the trading behavior of the market and is essential for the analysis of different types of trend present in the market \cite{tick}.

\subsection{Bid - Ask Spread}

Bid and Ask are the prices that buyers and sellers respectively are willing to transact at, the bid for the buying side, and the ask for the selling side. A transaction takes place when either a potential buyer is willing to pay the ask price, or a potential seller is willing to accept the bid price. The top bid refers to the maximum bid price in the order book and the top ask refers to the minimum ask price in the order book. The spread between the top bid and top ask price at any moment is called the bid-ask spread. The mid-price is the mean price of the top bid and top ask price \cite{bid_ask}.

Most of the standard trading algorithms work on the principle of mid-price prediction or mid-price movement prediction. However a big drawback of this technique can be seen from Fig \ref{baspread}. Clearly in case on the left, there is an increase in the mid-price of the product. But since we need to enter the market at the ask price (as a buyer) and exit at the bid price (as a seller), we are actually incurring a loss if we go through with this transaction. In case on the right, the movement of the price is large enough to cover the bid-ask spread and represents a profitable transaction.

\begin{figure}[h]
\centering
\includegraphics[width = 0.5\textwidth]{figures/baspread.png}
\caption[]{Two possible cases of increase in mid-price analyzed. Solid, blank and shaded represents the ask, mid and bid price of the product respectively.}
\label{baspread}
\end{figure}

We have diverted from the traditional approach of mid price prediction and instead focused on movement of the complete bid-ask spread so that we can directly fine-tune our model for profitability. This means our model predicts only those price movements which are substantial enough to cross the bid-ask spread. It should be noted that since we only consider change in price that cross the bid-ask spread as a "movement", predicting "no movement" does not mean that there was absolutely no movement in the price of the product. It just means that the movement was not substantial enough to cross the spread and thus, according to our model, was as useless as no actual movement in the price.

\subsection{Mean Reversion}
Mean reversion is a financial theory which suggests that the price of a stock tends to return towards its long running mean/average price over time \cite{bid_ask}. Trading on this strategy is done by noticing companies whose stock values have significantly moved away in some direction from its long running mean and thus is now expected to move in the opposite direction. Ignoring the erratic trading periods at the start and end of the day, this behavior in stock prices is evident in most of the stock markets across the world \cite{Chakraborty2011MarketMA}. The oscillating behavior of the price around some changing mean across the day as seen in Fig \ref{meanrev} is an example of Mean Reversion.

\begin{figure}[h]
\centering
\includegraphics[width = 0.5\textwidth]{figures/meanrev.png}
\caption[]{A snapshot of a full-day behavior of a random security picked from the training data}
\label{meanrev}
\end{figure}

Using mean reversion in stock price analysis involves both identifying the trading range for a stock (short-term information) and computing the evolution of the mean around which the prices will be oscillating (long-term information). Thus, being able to process extremely long sequences on multiple levels can allow our model to see a more complete picture of price movement and boost the prediction accuracy.

==> extras/05-proposed_solution.tex <==
\section{Proposed Solution}

The proposed pipeline contains a VLSTM network predicting the stock price movement followed by a financial model which places orders in the market based on the predicted movement. There has been a lot of research on what "features" to use for prediction or modeling \cite{Kearns_machinelearning, 1709.01268, doi:10.1111/j.1540-6261.1991.tb02683.x,1011.6402}. The common feature values like bid-ask spread, percentage change in price, weighted price etc. \cite{Kearns_machinelearning} and some specialized features like order imbalance \cite{imbalance} were among the few that we used in our model. The features are created such that they contain information regarding the local history, which depends on the look-back period as described in Section VII. From here on, the readers can assume the input to be a sequence of features.

\subsection{VLSTM Model}

The problem statement is modeled as a classification problem between three classes,
\begin{enumerate}
\item Increase in price that crosses bid-ask spread.
\item Decrease in price that crosses the bid-ask spread.
\item The change in price doesn't cross the bid-ask spread.
\end{enumerate}

We experiment with various combinations of the following LSTM levels \{1, 2, 5, 20, 100, 500, 2000, 5000\}. Each level has 2 LSTM cells stacked on top of each other with 16 hidden units each. The MLP layer used during training of individual LSTM levels contains 32 hidden units. The MLP layer used during final training for concatenated features also contains 32 hidden units. Activation functions used are ReLU at every hidden layer and softmax after the last layer. We also used Dropout layers to avoid overfitting. The error function used is Categorical Cross entropy with Adam optimizer.

Since every security in the market has a different frequency of activity, both look-back period for feature creation and range of future prediction is discussed in terms of number of ticks instead of absolute time. It can be interpreted as ignoring the concept of actual time and considering every tick in the life of a security as one second.

\subsection{Financial Model}

The prediction output provided by our model is a confidence score distribution between the 3 classes. We directly use the winning class prediction for accuracy evaluation. However, one can also define a threshold and only consider a prediction viable if the winning class confidence score is greater than the threshold. This threshold can thus work as a trade-off between participation and accuracy. For higher values of threshold, only prediction with very high confidence will remain viable, causing extremely low participation but with extremely high accuracy. On the other hand, lower threshold value would mean more participation but with lesser accuracy. 

Refer to Fig \ref{flowchart} for a a better understanding of the flow of the complete pipeline.

\begin{figure}[h]
\centering
\includegraphics[width = 0.5\textwidth]{figures/flowchart.png}
\caption[]{Flow of the complete pipeline. Feature generation is followed by VLSTM processing the input at various levels. The results are concatenated and passed through an MLP to provide confidence scores for different classes. These scores are then used by the financial module to take appropriate actions.}
\label{flowchart}
\end{figure}

==> extras/06-dataset.tex <==
\section{Dataset}

The dataset consists of tick by tick (tbt) data of a security with a frequency of over 15 million ticks across the day. Every tick contains the price and volume information of the last transaction and the top 5 levels of the order book of both the bid and ask side. The market behavior is erratic in the first few minutes after the market opens and in the last few minutes before it closes. So we removed the first 30 and the last 30 minutes of data to create a cleaner dataset.

For every LSTM level, we first changed the frequency of the input sequence and then divided it into sliding windows of length 100 each. This would mean around \begin{math}15,000,000/500=30000\end{math} datapoints of length 100 each for the level 500 LSTM and similarly varying amount of data for different levels of LSTMs. The complete data was then shuffled and divided into 60\% training, 10\% validation and 30\% test.

% The final dataset that we used for training and simulation contains around 200 filtered securities, with an average activity of around 70,000 ticks everyday. Thus we had approximately 70,000 * 200 = 14 million data points for every single day and a whole week's worth of similar data to work with.

==> tables/raw.tex <==
\begin{table}[h]
\scriptsize
\caption{Performance of VLSTMs at various levels}
\label{tab:vlstm}
\centering
\begin{tabular}{|cccccccc|c|c|}
\hline
\multicolumn{8}{|c|}{\textbf{VLSTM Levels}} & \textbf{Actionable} & \textbf{Weighted} \\
% \hline
1 & 2 & 5 & 20 & 100 & 500 & 2000 & 5000 & \textbf{Accuracy} (\%) & \textbf{F-score}\\
\hline
\checkmark & & & & & & & & 55.33 & 0.52\\
\hline
 & \checkmark & & & & & & & 54.12 & 0.53\\
\hline
 & & \checkmark & & & & & & 60.36 & 0.58\\
\hline
 & & & \checkmark & & & & & \textbf{61.37} & \textbf{0.59} \\
\hline
 & & & & \checkmark & & & & 56.97 & 0.57 \\
\hline
 & & & & & \checkmark & & & 53.63 & 0.54\\
\hline
 & & & & & & \checkmark & & 48.38 & 0.49\\
\hline
 & & & & & & & \checkmark & 50.96 & 0.50 \\
\hline
\hline
\checkmark & \checkmark & & & & & & & 58.98 & 0.57 \\
\hline
\checkmark & \checkmark & \checkmark & & & & & & 66.19 & 0.65\\
\hline
\checkmark & \checkmark & \checkmark & \checkmark & & & & & 71.41 & 0.68\\
\hline
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & & 75.54 & 0.75\\
\hline
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & 78.45 & 0.76 \\
\hline
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & 79.82 & 0.78 \\
\hline
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \textbf{80.70} & \textbf{0.79} \\
\hline
 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 80.29 & \textbf{0.79} \\
 \hline
  & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 79.68 & 0.78\\
 \hline
  & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 76.52 & 0.73 \\
\hline
  & & & & \checkmark & \checkmark & \checkmark & \checkmark & 70.69 & 0.71 \\
\hline
  & & & & & \checkmark & \checkmark & \checkmark & 57.46 & 0.54 \\
\hline
  & & & & & & \checkmark & \checkmark & 52.01 & 0.52\\
\hline
\end{tabular}
\end{table}

